Unbiased Teacher v2: Semi-supervised Object Detection for Anchor-free and Anchor-based Detectors

With the recent development of Semi-Supervised Object Detection (SS-OD) techniques, object detectors can be improved by using a limited amount of labeled data and abundant unlabeled data. However, there are still two challenges that are not addressed: (1) there is no prior SS-OD work on anchor-free detectors, and (2) prior works are ineffective when pseudo-labeling bounding box regression. In this paper, we present Unbiased Teacher v2, which shows the generalization of SS-OD method to anchor-free detectors and also introduces Listen2Student mechanism for the unsupervised regression loss. Specifically, we first present a study examining the effectiveness of existing SS-OD methods on anchor-free detectors and find that they achieve much lower performance improvements under the semi-supervised setting. We also observe that box selection with centerness and the localization-based labeling used in anchor-free detectors cannot work well under the semi-supervised setting. On the other hand, our Listen2Student mechanism explicitly prevents misleading pseudo-labels in the training of bounding box regression; we specifically develop a novel pseudo-labeling selection mechanism based on the Teacher and Student's relative uncertainties. This idea contributes to favorable improvement in the regression branch in the semi-supervised setting. Our method, which works for both anchor-free and anchor-based methods, consistently performs favorably against the state-of-the-art methods in VOC, COCO-standard, and COCO-additional.

==> figure/boundary_wise_reg_conf.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figure/pic/reg_conf.pdf}
    \caption{Comparison between the boundary-level and the box-level pseudo-labels. We aim to only enforce the unsupervised regression loss on the accurately predicted pseudo-boundaries (color in red).}
    \label{fig:boundary_wise_regconf}
\end{figure}


==> figure/centerness_bias_complete.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figure/pic/centerness_bias.pdf}
%     \caption{Illustration of centerness bias issue. 
%     We visualize the centerness, classification confidence, and IoU for each predicted bounding boxes (\textit{i.e.,} points in figure) in $15K$, $50K$, and $85K$ iterations.}
%     \label{fig:centerness_bias}
% \end{figure}


\begin{figure*}[t]
   \begin{picture}(0,180)
     \put(30,0){\includegraphics[width=0.9\linewidth]{figure/pic/centerness_bias.pdf}}
     \put(95,88){(a)}
     \put(245,88){(b)}
     \put(390,88){(c)}
    %  \put(70,-2){(c)}
     \put(245,-3){(d)}
    %  \put(320,-2){(e)}

   \end{picture}
    \caption{
    % \kevin{Should (b) use "Selection via Classification" instead of "Selection via Class Score" to make it consistent with (c)?}\yc{corrected it}
    \textbf{Centerness bias issue in semi-supervised anchor-free detectors}. 
    We analyze the detector in terms of its (b) mean average precision (mAP), (c) averaged scores of pseudo-boxes, and (d) correlation between centerness and classification score (y-axis) and IoU (colorization) for each predicted boxes. 
    % \zk{Added bolding  to highlight a-d here since you have a lot of text before it (which is confusing). May need more highlighting though. } \yc{thx}
    \textbf{(a)} Box score of some anchor-free detectors~\cite{tian2019fcos,zhang2020bridging} is derived by multiplying the centerness and the classification score.
    % \zk{Why not add this multiplication operation to the figure (a)?}.\yc{Added}
    \textbf{(b)} By using the box score to select pseudo-labels, the performance of the detector starts to degrade after $50$K training iterations. \textbf{(c)} We observe the box score of pseudo-boxes is dominated by the centerness score, which cannot precisely reflect whether the predicted boxes are foreground classes. As the predictions of the Teacher model is used as pseudo-labels for the Student model (\textit{i.e., pseudo-labeling}),
    the high-centerness background instances (points colored in dark blue in \textbf{(d)}) appear more frequently when the detector is trained longer. }
    \label{fig:centerness_bias_ceomplete}
\end{figure*}


==> figure/pseudo_anchor_free.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figure/pic/pseudo_anchor_free.pdf}
    \caption{Illustration of the center-sampling and localization-weighted classification labels, which is generated from the pseudo-labels.}
    \label{fig:pseudo_anchor_free}
\end{figure}

% \begin{figure}[t]
% \centering
% \subfloat[Heuristic-Based Level Assignment]{%
%   \includegraphics[width=.45\linewidth]{figure/pic/pseudo_anchor_free.pdf}%
%   \label{fig:heuristic}%
% }\qquad
% \subfloat[Training with All-Level Features]{%
%   \includegraphics[width=.45\linewidth]{figures/pic/all_level.png}%
%   \label{fig:all_level}%
% }
% \caption{Comparison between heuristic-based level assignment in Faster R-CNN and our proposed training with All-Level Features}
% \label{fig:fpn}
% \end{figure}

==> figure/pseudo_label_weakness.tex <==

\begin{figure}[t]
\centering
\subfloat[Unreliable label assignment]{%
  \includegraphics[width=.45\linewidth]{figure/pic/pseudo_anchor_free.pdf}%
  \label{fig:label_assignment}%
}\qquad
\subfloat[Box-level vs. Boundary-level pseudo-label for regression]{%
  \includegraphics[width=.45\linewidth]{figure/pic/reg_conf.pdf}%
  \label{fig:reg_label_level}%
}
\caption{(a) Label assignments of some existing anchor-free models~\cite{tian2019fcos,li2020generalized,li2020gflv2} are less robust to the localization noise (\textit{e.g.,} box center shift) in pseudo-boxes used in semi-supervised training. (b) Rather than box-level pseudo-label used in the existing SS-OD works, we aim to select the precisely predicted boundary and use boundary-level pseudo-labels for improving the bounding box regression branch.
\yc{Need to make a new figures to convey two major messages: anchor-free detectors and regression loss}
} 
\label{fig:fpn}
\end{figure}

==> impact.tex <==
% \section{Broader Impact}

% Our work discusses a fundamental problem in deep learning: data imbalance. Data imbalance can be safety-critical in many applications such as self-driving. Our approach allows an algorithm to give more attention to pedestrians and small obstacles. Additionally, our unified algorithm aims to provide stable performance under severe visual degradation which is also critical for safty considerations.   

==> table/analysis-breakdown-all.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Average precision (AP) breakdown of the model with and without our \proposedregmethod.}
\vspace{1mm}
\label{table:ap_breakdown}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccccc}
\toprule
        %   & \multicolumn{5}{c}{\textbf{Anchor-free detectors} on COCO-standard}  \\ \cline{2-6}
                           &  AP50 & AP55  & AP60  & AP65  & AP 70  & AP75& AP80 & AP85 & AP90 & AP95\\ \hline
No regression    & 31.53 & 29.71 & 27.34 & 24.64 &  21.38 & 17.55 & 13.27 & 8.33  & 3.45 & 0.35  \\ 
Confidence thresholding    & 32.59 & 30.78 & 28.59 & 26.19 &  23.05 & 19.64 & 15.61 & 10.47 & 5.06 & 0.58 \\ \hline
\proposedregmethod\    & 32.59 & 30.78 & 28.59 & 26.19 &  23.05 & 19.64 & 15.61 & 10.47 & 5.06 & 0.58 \\ \hline
% Absolute Improvement (mAP) & +1.06 & +1.07 & +1.25 & +1.56 &  +1.67 & +2.09 & +2.34 & +2.14 & +1.61 & +0.23 \\ 
Relative Improvement (\%)  & \textcolor{myblue}{+3.36} & \textcolor{myblue}{+3.60} & \textcolor{myblue}{+4.57} & \textcolor{myblue}{+6.29} &  \textcolor{myblue}{+7.81} & \textcolor{myblue}{+11.91} & \textcolor{myblue}{+17.63} & \textcolor{myblue}{+25.69} & \textcolor{myblue}{+46.67} & \textcolor{myblue}{+65.71} \\ 
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table}

==> table/analysis-margin.tex <==
% \begin{table}[h]
% \centering
% % \renewcommand{\arraystretch}{1.3}
% \caption{Ablation study of varying margin between the localization uncertainties of Teacher and Student $\sigma$ in the case of \textit{COCO-standard} 1\%. FCOS is used as the model for all results below.}
% \label{table:margin}
% \resizebox{0.6\linewidth}{!}{%
% \begin{tabular}{ccccc}
% \toprule\hline
%  $\sigma$   & 0.0   &  0.1   & 0.2   & 0.3   \\ \hline
%  mAP         & 19.93 &  20.19 & 19.84 & 18.80 \\ \hline
% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}[h]
\centering
% \renewcommand{\arraystretch}{1.3}
\caption{Ablation study of varying margin between the localization uncertainties of Teacher and Student $\sigma$ in the case of \textit{COCO-standard} 1\%. Faster-RCNN is used as the model for all results below.}
\label{table:margin}
\resizebox{0.7\linewidth}{!}{%
\begin{tabular}{cccccc}
\toprule
 $\sigma$   & 0.0   &  0.1   & 0.2   & 0.3  & 0.4 \\ \hline
 mAP        & 22.15 &  22.27 & \textbf{22.73} & 22.57 & 21.91 \\ 
\bottomrule
\end{tabular}
}
\end{table}

==> table/analysis-unsup_reg.tex <==
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \caption{Ablation study of unsupervised regression loss.}
% % We ablate different unsupervised regression loss on our anchor-free model, and our~\proposedregmethod\ can perform favorably against the existing unsupervised regression loss.}
% % \yc{I didn't change this, as the ablation of modifications to anchor-free models are verified in Figure~\ref{fig:centerness_bias} and \ref{fig:label_assignment_results}}
% \vspace{1mm}
% \label{table:ablate_ureg}
% \resizebox{0.5\linewidth}{!}{%
% \begin{tabular}{cccc}
% \toprule
%           & \multicolumn{3}{c}{COCO-standard 1\% }  \\ \cline{2-4}
% \multirow{2}{*}{Methods}      & \proposedregmethod &  \multirow{2}{*}{Confidence thresholding}    & \multirow{2}{*}{No regression}   \\ 
%           & (Ours) &   &       \\ \hline
%             &  19.28            &     18.27          &   17.79   \\ 
% \bottomrule
% \end{tabular}
% }
% \vspace{-3mm}
% \end{table}




% Vertical version
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \caption{Ablation study of unsupervised regression loss.}
% % We ablate different unsupervised regression loss on our anchor-free model, and our~\proposedregmethod\ can perform favorably against the existing unsupervised regression loss.}
% % \yc{I didn't change this, as the ablation of modifications to anchor-free models are verified in Figure~\ref{fig:centerness_bias} and \ref{fig:label_assignment_results}}
% \label{table:ablate_ureg}
% \begin{tabular}{c|c}
% \toprule
%                   & mAP   \\\hline
% No Regression      & 17.79 \\
% Conf. Thresholding & 18.27 \\
% ~\proposedregmethod   (Ours) & 19.56\\
% \bottomrule
% \end{tabular}
% \vspace{-3mm}
% \end{table}


\begin{table*}[!t]
\begin{minipage}[t]{0.68\textwidth}
\captionof{table}{ {Results of the {anchor-free model (FCOS)} on \textit{VOC}}.}  
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccl}
\Xhline{2\arrayrulewidth}
          & \multicolumn{4}{c}{\textbf{Anchor-free detectors} on VOC}  \\ \cline{2-5}
 & Models & Labeled & Unlabeled  & \multicolumn{1}{c}{$AP_{50:95}$} \\ \hline
 Supervised& \scriptsize{FCOS-R50}  & VOC07 & None & 41.53  \\\hline
% Supervised (from STAC)& \scriptsize{ResNet50-FPN}  & VOC07 & None & 42.60  \\ 
% CSD & \scriptsize{ResNet101-R-FCN}  & \multirow{3}{*}{VOC07} & \multirow{3}{*}{VOC12}   & -   \\ 
STAC~\cite{sohn2020simple} & \scriptsize{FCOS-R50} &  \multirow{3}{*}{VOC07} & \multirow{3}{*}{VOC12}  & 44.47 \scriptsize{\textcolor{myblue}{(+2.94)}}  \\
Unbiased Teacher~\cite{liu2021unbiased} & \scriptsize{FCOS-R50} &   &   & 49.50 \scriptsize{\textcolor{myblue}{(+7.97)}}  \\
Ours & \scriptsize{FCOS-R50} & &  & \textbf{51.47 \scriptsize{\textcolor{myblue}{(+9.94)}}}\\ \hline
% CSD & \scriptsize{ResNet101-R-FCN} &  \multirow{3}{*}{VOC07} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VOC12\\ +\\ \textit{COCO20cls}\end{tabular}}  & -   \\ 
STAC~\cite{sohn2020simple} & \scriptsize{FCOS-R50} &  \multirow{3}{*}{VOC07} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VOC12 \\+\\ \textit{COCO20cls}\end{tabular}}  & 44.89 \scriptsize{\textcolor{myblue}{(+3.36)}}  \\
Unbiased Teacher~\cite{liu2021unbiased} & \scriptsize{FCOS-R50} &  &  & 51.15 \scriptsize{\textcolor{myblue}{(+9.62)}}  \\
Ours & \scriptsize{FCOS-R50}  & &   & \textbf{52.95 \scriptsize{\textcolor{myblue}{(+11.42)}}} \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
% We observe that the Baseline gets relatively higher as the domain difference gets larger.
\label{table:voc}
\end{minipage}
\hfill
\begin{minipage}[t]{0.3\textwidth}
\captionof{table}{Ablation study of unsupervised regression loss. All methods use FCOS in COCO-standard 1$\%$.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cc}
\toprule
                  & mAP   \\\hline
No Regression      & 17.79 \\
Conf. Thresholding & 18.27 \\
~\proposedregmethod\  (Ours)               & \textbf{19.56}\\
\bottomrule
\end{tabular}
}
\label{table:ablate_ureg}
\end{minipage}
\end{table*}

==> table/analysis_breakdown.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Average precision (AP) breakdown of the model with and without our \proposedregmethod.}
\vspace{1mm}
\label{table:ap_breakdown}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccccc}
\toprule
        %   & \multicolumn{5}{c}{\textbf{Anchor-free detectors} on COCO-standard}  \\ \cline{2-6}
                           &  AP50 & AP55  & AP60  & AP65  & AP 70  & AP75& AP80 & AP85 & AP90 & AP95\\ \hline
w/o \proposedregmethod\    & 31.53 & 29.71 & 27.34 & 24.64 &  21.38 & 17.55 & 13.27 & 8.33  & 3.45 & 0.35  \\ 
w/  \proposedregmethod\    & 32.59 & 30.78 & 28.59 & 26.19 &  23.05 & 19.64 & 15.61 & 10.47 & 5.06 & 0.58 \\ \hline
% Absolute Improvement (mAP) & +1.06 & +1.07 & +1.25 & +1.56 &  +1.67 & +2.09 & +2.34 & +2.14 & +1.61 & +0.23 \\ 
Relative Improvement (\%)  & \textcolor{myblue}{+3.36} & \textcolor{myblue}{+3.60} & \textcolor{myblue}{+4.57} & \textcolor{myblue}{+6.29} &  \textcolor{myblue}{+7.81} & \textcolor{myblue}{+11.91} & \textcolor{myblue}{+17.63} & \textcolor{myblue}{+25.69} & \textcolor{myblue}{+46.67} & \textcolor{myblue}{+65.71} \\ 
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table*}


==> table/analysis_dataaug_l2s.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{Ablation study on Listen2student and scale jitter. Note that we experiment on COCO-standard with $10\%$ supervision. Faster-RCNN is used as the model for all results below.}
\label{table:ablation_scale_jitter}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{ccc}
\toprule
Listen2student   & Scale jitter & mAP  \\ \specialrule{1pt}{1pt}{1pt}
-                & - & 30.91   \\ 
\checkmark       & - & \textbf{32.18}   \\ \midrule
-                & \checkmark & 31.83   \\ 
\checkmark       & \checkmark & \textbf{33.55}   \\ 
\bottomrule
\end{tabular}
}
\end{table}


==> table/anchorfree_mod_complete.tex <==
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \caption{}
% \label{table:pseudo-label-select}
% \resizebox{0.8\linewidth}{!}{%
% \begin{tabular}{ccc}
% \toprule
% Standard  & Use Cls. score & mAP \\ \specialrule{1pt}{1pt}{1pt}
% - & - &  42.50     \\ 
% \checkmark & - & 43.23  \\ 
% - & \checkmark &  44.48     \\ 
% % \checkmark & \checkmark &  43.31     \\ 

% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
% \textcolor{red}{
% Box selection based on box scores is worse than classification scores in the semi-supervised setting, while this trend is contrary in the fully-supervised setting (for NMS box selection).
% }
Pseudo-box selection based on classification scores is more effective than pseudo-box selection based on box score (which contains centerness score) in COCO-additional. 
All results are based on FCOS~\cite{tian2019fcos}.}
\label{table:boxscore_cocoadd}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{cccc}
\toprule
                           & Class. score & Box score & $\Delta$ \\ \specialrule{1pt}{1pt}{1pt}
COCO-additional            & 44.48 & 42.50 &  \textbf{\textcolor{red}{-1.98}}     \\ 
\bottomrule
\end{tabular}
}
\end{table}


\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
Using center-sampling leads to a worse accuracy in COCO-additional. All results are based on FCOS~\cite{tian2019fcos}.
}
\label{table:centersample_cocoadd}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc}
\toprule
                           & w/o Center-Sampling & w/ Center-Sampling & $\Delta$ \\ \specialrule{1pt}{1pt}{1pt}
COCO-additional            & 43.23 & 42.50 &  \textbf{\textcolor{red}{-0.53}}     \\ 
\bottomrule
\end{tabular}
}
\vspace{3mm}
\end{table}


==> table/augment.tex <==
\begin{table}[ht]
    \centering
    \caption{
Detail of data augmentations. Probability in the table indicates the probability of applying the corresponding image process.}
    \label{table:data_aug_parameter}
    \vspace{3mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccl}
\toprule\toprule
\multicolumn{4}{c}{\textbf{Weak Augmentation}}\\
\midrule
Process& Probability & Parameters& \multicolumn{1}{c}{Descriptions}\\
\midrule
Horizontal Flip & 0.5& -& \multicolumn{1}{c}{None}\\ \midrule \midrule
\multicolumn{4}{c}{\textbf{Strong Augmentation}}\\ \midrule
Process         & Probability & Parameters& \multicolumn{1}{c}{Descriptions}\\\midrule
Color Jittering & 0.8                     & \begin{tabular}[c]{@{}c@{}}(brightness, contrast, saturation, hue)\\ = (0.4, 0.4, 0.4, 0.1)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Brightness factor is chosen uniformly from {[}0.6, 1.4{]},\\ contrast factor is chosen uniformly from {[}0.6, 1.4{]},\\ saturation factor is chosen uniformly from {[}0.6, 1.4{]},\\ and hue value is chosen uniformly from {[}-0.1, 0.1{]}.\end{tabular} \\ \midrule
Grayscale       & 0.2                     & None                                                                                                       & \multicolumn{1}{c}{None}                                                                                                                                                                                                                                                                                    \\  \midrule
GaussianBlur    & 0.5                     & (sigma\_x, sigma\_y) = (0.1, 2.0)                                                                        & Gaussian filter with $\sigma_x=0.1$ and $\sigma_y=2.0$ is applied.                                                                                                                                                                                                                   \\ \midrule
CutoutPattern1  & 0.7                     & scale=(0.05, 0.2),  ratio=(0.3, 3.3)                                                                     & \begin{tabular}[c]{@{}l@{}}Randomly selects a rectangle region in an image\\  and erases its pixels. We refer the detail in~\cite{zhong2017random}.\end{tabular}                                                                                                                                             \\ \midrule
CutoutPattern2  & 0.5                     & scale=(0.02, 0.2), ratio=(0.1, 6)                                                                        & \begin{tabular}[c]{@{}l@{}}Randomly selects a rectangle region in an image\\  and erases its pixels. We refer the detail in~\cite{zhong2017random}.\end{tabular}                                                                                                                                             \\ \midrule
CutoutPattern3  & 0.3                     & scale=(0.02, 0.2), ratio=(0.05, 8)                                                                       & \begin{tabular}[c]{@{}l@{}}Randomly selects a rectangle region in an image\\  and erases its pixels. We refer the detail in~\cite{zhong2017random}.\end{tabular}
\\
\bottomrule\bottomrule
\end{tabular}}
\end{table}


==> table/coco_additioal_anchor_free.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{\textcolor{black}{
    {Experimental results of the anchor-free model (FCOS-ResNet50) on \textit{COCO-additional}}.
    Note that 1x represents 90K training iterations, and $N$x represents $N\times$90K training iterations. 
    }
    }
\label{table:mscoco-add}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
          & \multicolumn{6}{c}{\textbf{Anchor-free detectors} on COCO-additional}  \\ \cline{2-8}
          & Supervised (1x) & Supervised (3x) & CSD (3x)   & STAC (3x)  &Unbiased Teacher (3x) & Ours (3x)  & Ours (4x)   \\ \hline
$AP^{50:95}$&  37.10 & 37.29 & 36.70 \scriptsize{\textcolor{red}{(-0.59)}}  &   38.06 \scriptsize{\textcolor{myblue}{(+0.77)}}   & 39.84 \scriptsize{\textcolor{myblue}{(+2.55)}}& \textbf{44.02\scriptsize{\textcolor{myblue}{(+6.73)}}} & \textbf{44.48 \scriptsize{\textcolor{myblue}{(+7.19)}}}    \\ 

\bottomrule
\end{tabular}
}
\end{table*}


==> table/data_aug.tex <==
\begin{table*}[ht]
    \centering
    \renewcommand{\arraystretch}{1.3}
    \caption{
    Meanings and values of the hyper-parameters used in \textbf{FCOS} in experiments.
    }
    \label{table:hyperparameters_fcos}
    \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{llccc}
        \toprule
        Hyper-parameter & Description & \textit{COCO-standard}  & \textit{VOC} & \textit{COCO-additional} \\
        \midrule
        $\tau$ & Class. confidence threshold     & 0.5    & 0.5 & 0.5\\
        % $\sigma$ & Margin between Teacher and Student     & 0.2   & 0.2 & 0.2\\
        % $\sigma_s$ & Student regression threshold     & 0.3 & 0.3 & 0.3 \\
        $\lambda^{cls}_{u}$ & Unsupervised loss weight for classification  & 3      & 3 & 2\\
        $\lambda^{reg}_{u}$ & Unsupervised loss weight for regression  & 0.2      & 0.2 & 0.2  \\
        $\alpha$ & EMA rate                        & 0.9999 & 0.9999 & 0.9999\\
        $b_{l}$ & Batch size for labeled data      & 8 & 16 & 32\\
        $b_{u}$ & Batch size for unlabeled data    & 8 & 16 & 32\\
        $\gamma$ & Learning rate                  & 0.01 & 0.01 & 0.01\\
        \bottomrule
    \end{tabular}
}
\end{table*}


\begin{table*}[ht]
    \centering
    \renewcommand{\arraystretch}{1.3}
    \caption{
    Meanings and values of the hyper-parameters used in \textbf{Faster-RCNN} in experiments.
    }
    \label{table:hyperparameters_fasterrcnn}
    \resizebox{0.7\textwidth}{!}{
    \begin{tabular}{llccc}
        \toprule
        Hyper-parameter & Description & \textit{COCO-standard}& \textit{VOC}  & \textit{COCO-additional} \\
        \midrule
        $\delta$ & Confidence threshold               & 0.7 & 0.7 & 0.7\\
        % $\sigma$ & Margin between Teacher and Student & 0.2 & 0.2  & 0.2 \\
        % $\sigma_s$ & Student regression threshold     & 0.3 & 0.3 & 0.3 \\
        $\lambda^{cls}_{u}$ & Unsupervised loss weight for classification  & 4 & 2& 2\\
        $\lambda^{reg}_{u}$ & Unsupervised loss weight for regression  & 1.0 & 1.0 & 1.0\\
        $\alpha$ & EMA rate                           & 0.9996 & 0.9996 & 0.9996\\
        $b_{l}$ & Batch size for labeled data         & 8/32    & 8    & 32 \\
        $b_{u}$ & Batch size for unlabeled data       & 8/32/40 & 8    & 32 \\
        $\gamma$ & Learning rate                      & 0.01    & 0.01 & 0.01\\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> table/rebuttal/centernet.tex <==

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{\textbf{Semi-supervised object detection with CenterNet~\cite{zhou2019objects}.} We use $1\%$ data as the labeled set and the remaining data as the unlabeled set. }
\label{table:centernet}
\vspace{-3mm}
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{cc}
\toprule
Methods & mAP   \\
\midrule
CenterNet ($1\%$; Supervised-only)          &  8.17 \\
CenterNet ($1\%$; Unbiased Teacher)    & 14.81 \\
CenterNet ($1\%$; Ours)                & 20.31 \\

\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}



==> table/rebuttal/iou.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{\textbf{Comparison between IoU scores and our method.} We experiment on $0.5$\% COCO-standard setting. }
\label{table:iou}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{cccc}
\toprule
 Method  & No regression  &  Estimated IoU scores &  Our method           \\
 \midrule
mAP & 17.79 & 18.28 & 19.56\\
\bottomrule
% \midrule
% Student Error $||\tilde{d}_s - d_g ||$ &  0.717 & 0.949 & 1.060 & 1.135  & 1.193 & 1.248 \\
% Teacher Error $||\tilde{d}_t - d_g ||$ &  0.580 & 0.701 & 0.724 & 0.708  & 0.676 & 0.631 \\
% Error Difference  &  \textcolor{red}{-0.137} & \textcolor{red}{-0.248} & \textcolor{red}{-0.336}  & \textcolor{red}{-0.427}  & \textcolor{red}{-0.517} & \textcolor{red}{-0.617} \\
\end{tabular}
}
\vspace{-3mm}
\end{table}

==> table/rebuttal/relateive_uncertainty.tex <==
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \caption{\textbf{Correlation between beneficial cases and the margin between Teacher's uncertainties and Student uncertainties.} We select the instances where $\delta_t + \sigma \leq \delta_s$ and vary the margin size $\sigma$.
% When the margin $\sigma$ between Teacher's uncertainty and Student's uncertainty becomes larger, the percentage of beneficial cases in pseudo-labels increases. This also leads to larger gap between Teacher averaged error and Student averaged error, which indicates the Teacher's prediction can be more beneficial to  }
% \vspace{1mm}
% \label{table:percentage_beneficial}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{cc|ccc}
% \toprule
% \multirow{2}{*}{$\sigma$} & Percentage of & Teacher Avg. Error & Student Avg. Error & \multirow{2}{*}{Error Gap} \\
%  & Beneficial Cases & $||\tilde{d}_t - d_g ||$ & $||\tilde{d}_s - d_g ||$ &     \\
% \midrule
% 0        & 55.9                           & 0.580                 & 0.717   &   0.137         \\
% 0.1      & 60.76                          & 0.701                 & 0.949   &   0.248        \\
% 0.2      & 63.72                          & 0.724                 & 1.060   &   0.336        \\
% 0.3      & 66.58                          & 0.708                 & 1.135   &   0.427        \\
% 0.4      & 69.27                          & 0.676                 & 1.193   &   0.517        \\
% 0.5      & 72.17                          & 0.631                 & 1.248   &   0.617       \\
% \bottomrule
% \end{tabular}
% }
% \vspace{-3mm}
% \end{table}


\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{\textbf{Correlation between misleading/beneficial cases and the margin $\sigma$ between Teacher uncertainties $\delta_t$ and Student uncertainties $\delta_s$.} We select the pseudo-labels where $\delta_t + \sigma \leq \delta_s$ and compute the percentage of beneficial cases.
When the margin $\sigma$ becomes larger, the percentage of beneficial cases in pseudo-labels increases.}
\vspace{-3mm}
% This also leads to larger gap between Teacher averaged error and Student averaged error, which indicates the Teacher's prediction can be more beneficial to  }
\label{table:percentage_beneficial}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|cccccc}
\toprule
 Margin b/w Teacher and Student uncertainties $\sigma$ &0        & 0.1& 0.2&0.3&0.4  &0.5          \\
\midrule
Percentage of \textbf{Misleading} Cases (\%)& 44.10     & 39.24 & 36.28& 33.42 & 30.73 & 27.83       \\
Percentage of \textbf{Beneficial} Cases (\%)& 55.90     & 60.76 & 63.72& 66.58 & 69.27 & 72.17       \\
% \midrule
% Student Error $||\tilde{d}_s - d_g ||$ &  0.717 & 0.949 & 1.060 & 1.135  & 1.193 & 1.248 \\
% Teacher Error $||\tilde{d}_t - d_g ||$ &  0.580 & 0.701 & 0.724 & 0.708  & 0.676 & 0.631 \\
% Error Difference  &  \textcolor{red}{-0.137} & \textcolor{red}{-0.248} & \textcolor{red}{-0.336}  & \textcolor{red}{-0.427}  & \textcolor{red}{-0.517} & \textcolor{red}{-0.617} \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table}

==> table/rebuttal/uncertainty_bene_mislead.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{The percentage of beneficial cases in pseudo-labels increases when the margin $\sigma$ between Teacher's uncertainty and Student's uncertainty becomes larger.  }
\vspace{1mm}
\label{table:percentage_beneficial}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc}
                & Teacher Avg. Uncertainty $\delta_t$ & Student Avg. Uncertainty $\delta_s$ & Difference \\
Misleading      & 0.39               & 0.46                 & 0.07              \\
Beneficial      & 0.32               & 0.52                 & 0.23              \\
\end{tabular}
}
\vspace{-3mm}
\end{table}

==> table/voc_anchor_free.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
    Results of the \textbf{anchor-free model (FCOS)} on \textit{VOC}. % comparing with STAC~\cite{sohn2020simple} and Unbiased Teacher~\cite{liu2021unbiased}. 
    % Note that the results of Supervised are from STAC.
    % Note that we report the CSD result from the original paper, and they use ResNet101-R-FCN as feature backbone. For the remaining methods including the supervised baseline, we use ResNet50-FPN as feature backbone. 
    }
\label{table:voc}
\resizebox{\linewidth}{!}{%
\begin{tabular}{llccl}
\Xhline{2\arrayrulewidth}
 & Models & Labeled & Unlabeled  & \multicolumn{1}{c}{$AP_{50:95}$} \\ \hline
 Supervised& \scriptsize{FCOS-R50}  & VOC07 & None & 41.53  \\\hline
% Supervised (from STAC)& \scriptsize{ResNet50-FPN}  & VOC07 & None & 42.60  \\ 
% CSD & \scriptsize{ResNet101-R-FCN}  & \multirow{3}{*}{VOC07} & \multirow{3}{*}{VOC12}   & -   \\ 
STAC~\cite{sohn2020simple} & \scriptsize{FCOS-R50} &  \multirow{3}{*}{VOC07} & \multirow{3}{*}{VOC12}  & 44.47 \scriptsize{\textcolor{myblue}{(+2.94)}}  \\
Unbiased Teacher~\cite{liu2021unbiased} & \scriptsize{FCOS-R50} &   &   & 49.50 \scriptsize{\textcolor{myblue}{(+7.97)}}  \\
Ours & \scriptsize{FCOS-R50} & &  & \textbf{56.71 \scriptsize{\textcolor{myblue}{(+15.13)}}}\\ \hline
% CSD & \scriptsize{ResNet101-R-FCN} &  \multirow{3}{*}{VOC07} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VOC12\\ +\\ \textit{COCO20cls}\end{tabular}}  & -   \\ 
STAC~\cite{sohn2020simple} & \scriptsize{FCOS-R50} &  \multirow{3}{*}{VOC07} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}VOC12 \\+\\ \textit{COCO20cls}\end{tabular}}  & 44.89 \scriptsize{\textcolor{myblue}{(+3.36)}}  \\
Unbiased Teacher~\cite{liu2021unbiased} & \scriptsize{FCOS-R50} &  &  & 51.15 \scriptsize{\textcolor{myblue}{(+9.62)}}  \\
Ours & \scriptsize{FCOS-R50}  & &   & \textbf{57.91 \scriptsize{\textcolor{myblue}{(+16.38)}}} \\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
% \vspace{-3mm}
\end{table}

